Real-Time Point Cloud Fusion of Multi-LiDAR Infrastructure Sensor Setups with Unknown Spatial Location and Orientation

The use of infrastructure sensor technology for traffic detection has already been proven several times. However, extrinsic sensor calibration is still a challenge for the operator. While previous approaches are unable to calibrate the sensors without the use of reference objects in the sensor field of view (FOV), we present an algorithm that is completely detached from external assistance and runs fully automatically. Our method focuses on the high-precision fusion of LiDAR point clouds and is evaluated in simulation as well as on real measurements. We set the LiDARs in a continuous pendulum motion in order to simulate real-world operation as closely as possible and to increase the demands on the algorithm. However, it does not receive any information about the initial spatial location and orientation of the LiDARs throughout the entire measurement period. Experiments in simulation as well as with real measurements have shown that our algorithm performs a continuous point cloud registration of up to four 64-layer LiDARs in real-time. The averaged resulting translational error is within a few centimeters and the averaged error in rotation is below 0.15 degrees.

==> social_media_post.tex <==
Check out our latest paper "Real-Time  Point  Cloud  Fusion  of  Multi-LiDAR  Infrastructure Sensor Setups  with  Unknown  Spatial  Location  and  Orientation" (arXiv) by @Laurent Kloeker and @Christian Kotulla. We are glad to announce that the work is accepted for presentation at this year's 23rd Intelligent Transportation Systems Conference (#IEEE #ITSC 2020).

It combines multiple interesting aspects of #computervision in #autonomousvehicles:

               • 360° camera-based environment perception in a transformed bird's eye view
               • Deep Learning-based distance estimation using mono-cameras
               • Learning from simulations and transfer to the real world
               • Uncertainty estimation for occluded areas

The video shows a semantic segmentation of a scene in bird's eye view, which is computed by a neural network from the images of multiple vehicle-mounted cameras. The network is trained with synthetic data, but can also be applied to real-world data as described in the paper.

Head over to the GitHub repository to try out our approach now! We provide a TensorFlow implementation and two synthetic datasets.
#ieee #itsc #

